Behavior Sequence Transformer for E-commerce Recommendation in Alibaba

Deep learning based methods have been widely used in industrial recommendation systems (RSs). Previous works adopt an Embedding&MLP paradigm: raw features are embedded into low-dimensional vectors, which are then fed on to MLP for final recommendations. However, most of these works just concatenate different features, ignoring the sequential nature of users' behaviors. In this paper, we propose to use the powerful Transformer model to capture the sequential signals underlying users' behavior sequences for recommendation in Alibaba. Experimental results demonstrate the superiority of the proposed model, which is then deployed online at Taobao and obtain significant improvements in online Click-Through-Rate (CTR) comparing to two baselines.

==> behemoth.tex <==
\section{Introduction}
Traditional approaches for CF-based recommender systems have mostly relied on elementary co-occurrence statistics or
matrix factorization. However, over the past few years, there has been a shift to build recommendation models that rely
on vectorial representations of discrete data, i.e. embeddings. There are a number of reasons why this has in general
been considered advantageous over traditional approaches:
\begin{itemize}
    \item Once embeddings for all items have been obtained, similarities for item (user, etc.) pairs may easily be
        computed, even if there is no co-occurrence data available.
    \item If implemented properly, embedding based methods may allow for cold start recommendation of new items.
    \item All recommendation and search related objects may be embedded into the same semantic vector space, creating
        the possibility for the development of a unified search and recommendation framework on top of vectorial
        representations.
    \item Vectorial representations (sparse or dense) of objects such as items, user, categories, types, etc. are  in
        general better suited to be fed into deep neural networks, thus possibly allowing for the design of much more sophisticated
        models (consider e.g.  Wide and Deep Ranking or multimodal embedding models \cite{wideanddeep,youtube}).
\end{itemize}

Thus, a number of "x2vec" models have been proposed over the recent years, where "x" has stood for objects like
as "Item" \cite{item2vec}, "(Meta-)Product" \cite{mp2v}, "Metapath" \cite{metapath2vec}, etc. This development has
mainly been fueled by the realization that the original word2vec algorithm by Mikolov \cite{word2vec} may successfully be
generalized and deployed in non-NLP contexts, such as recommender systems or social network analysis
\cite{deepwalk,node2vec,metapath2vec,alikdd2}. 
Virtually all of these methods are implemented using a Skip-Gram model in conjunction with negative sampling. We hence summarize all of these methods under the term "SGNS-type algorithms".

In this article we present how SGNS-type algorithms have successfully been applied for generating high-quality recommendations in the Taobao Mobile App. In particular, we describe how they can easily be used to incorporate additional discrete product features ("side information"), further increasing the overall recommendation performance. Such "context enriched" SGNS-type algorithms have been applied successfully for instance in \cite{mp2v} \cite{alikdd2}. 

Our key contributions can be summarized as follows:
\begin{enumerate}
\item We show how the Target Negative Sampling (TNS) method \cite{dsgns} can be used obtain joint embeddings for very large (possibly billion-scale) sets of items and side information features. In particular, we show the necessity of suitable partitioning and averaging strategies that are needed to address the imbalance problems caused by a highly skewed distribution of item and side information features in the training data (Sections \ref{sect:scaling} and \ref{sect:asymp2vtns}).
\item We present the ASYMP2V model, which we train in production using random walks on a graph of roughly 500 millions products with billions of edges.  This model can be considered as a  simplified, yet highly effective, variation of the Meta-Product2Vec \cite{mp2v} model, allowing for competitive performance, while still being efficient enough to be retrained regularly in a matter of hours (Section \ref{sect:asymp2v}).  
\item We develop a semi-formal theoretical argument for the effectiveness of SGNS-type algorithms and show how it can be used to explain the superior performance of "context enriched" SGNS-type algorithms as in \cite{mp2v} or \cite{alikdd2}. Furthermore, a similar argument allows us to theoretically justify our heuristics for deriving cold start recommendations for new items from side information embeddings (Sections \ref{sect:sgns} and \ref{sect:coldstart}).
\item \textbf{TODO: If one paper: add Behemoth platform description and engineering challenges.}
\end{enumerate} 
This article is structured as follows: In Section \ref{sect:first} we first review some elementary theory in and then provide a semi-formal argument explaining the effectiveness of SGNS-type algorithms using a formulation of trained embedding vectors in terms of a product of learned co-occurence statistics and the initial data. Afterwards we describe a relatively known general approach to incorporate side information into SGNS-type algorithms using context enrichment. The section concludes with a basic description of the TNS method from \cite{dsgns}.

In Section \ref{sect:asymp2v} we describe the ASYMP2V model, how it can be applied for cold-start recommendation and other transfer tasks, as well as describe challenges and solutions when combining ASYMP2V (or similar models) with a distributed training algorithm based on TNS. Before concluding this article we present several case studies both using public, as well as proprietary datasets. The case studies contain results regarding both the recommendation performance, as well as the computational efficiency of our implementation.

\section{Product Recommendation using Graph Embedding with Side Information}
\label{sect:first}
Our starting point is a graph $G$ modeling user-item interactions. Typically, such a graph is obtained from  recorded user actions. In the context of many recommender systems, particularly those used in online shops or similar environments, one considers an item to item (i2i) graph $G$ of the form 
\[ 
G = (\mathcal{V}, \mathcal{E}), \quad \mathcal{V} = \{V : V \text{ item (e.g. on Taobao)}\}, \quad \vert \mathcal{V} \vert = N,
\]
where the graph's edges $\mathcal{E}$ are defined by 
\[
    \quad \mathcal{E} = \{(U,V,p(U,V)) : 0 \leq p(U,V)  \leq 1\}.
\]
Here, $p(U,V)$ represents the probability of an arbitrary user clicking on item $U$, conditioned on him or her
currently looking at item $V$. We can thus model user behavior as a time discrete Markov chain $V^{(k)}$ on $G$ with transition
probabilities $p(U,V)$. Hence, $V^{(k)}$
corresponds to the $k$-th item looked at by a user who started his online shopping session at an initial item $V^{(0)}$. 

Our ultimate goal is now  to find an embedding
$f:\mathcal{V} \rightarrow \mathbbm{R}^{d}$ such that
\[
    \sigma(s(f(U), f(V))) \approx \min_{k > 0} P(V^{(k)} = U  \mid  V^{(0)} = V),
\]
where $\sigma$ is the sigmoid function $\sigma(x) = \frac{1}{1+\exp(-x)}$ and  $s: \mathbbm{R}^{d}  \times \mathbbm{R}^{d} \rightarrow \mathbbm{R}$ is some similarity measure, such as the
cosine similarity $s(u,v) = u^T v / \|u\|_2 / \|v\|_2$ or the standard Euclidean metric $s(u,v) = \| u - v\|_2$. Once we
have obtained embeddings for all items, the similarity between any two items can be calculated and a recommendation based on
an initial "trigger" item may simply be realized by querying for the top-k nearest neighbours its embedding vector.

Having collected a sufficiently large number of realizations of the process $V^{(k)}$, we may interpret the entirety of the collected
item sequences as a text corpus and recast
the above graph embedding problem as a word embedding problem a la word2vec \cite{word2vec}. Hence, we may obtain an embedding $f$
by simply feeding a set of item sequences into a standard word embedding algorithm.

To obtain training data, that is concrete realizations of the process $V^{(k)}$, one could construct the graph $G$ and estimate transition probabilities
using basic statistical analysis
of logged user actions. Yet, for concrete applications it may not even necessary to construct the whole graph $G$: When there already is a large number of recorded user
actions available, then it may actually be preferable to directly use real user sequences as training data, as this might
prevent introducing an unintended bias. On the other hand, artificially generated sequences might prove useful for
introducing a specific, application dependent, bias into the generated sequences.

\begin{figure*}[hbpt]
\center
\includegraphics[width=0.85\textwidth]{figures/sequences.png}
    \caption{Product embeddings may be obtained by directly utilizing user-item sequences (left) or indirectly via first
    constructing an i2i graph (middle) and then generating sequences of items using a random walk on this graph (right).
    The final sequences are then fed into an SGNS-type algorithm.}
\label{fig:sequences}
\end{figure*}

\subsection{SGNS-type Algorithms}
\label{sect:sgns}
Assuming that we are given sequences of items, which have either been obtained directly from logged user behavior or
generated by a random walk, we can now apply an SGNS-type algorithm (Skip-Gram with Negative Sampling) in order to learn
the embedding $f$ \cite{word2vec, deepwalk, node2vec, metapath2vec, mp2v}.

Skip-gram models have first been used in the context of word embeddings (See e.g. the seminal work of Mikolov \cite{word2vec}) and
later been used for graph embedding problems \cite{deepwalk, node2vec} by learning an embedding from a "corpus" of random walk
or similarly generated node sequences (See also \cite{mit} for a more rigorous justification of this approach). 

We briefly review the basics of SGNS-type algorithms: Given a sequence of items (words, nodes, resp.) $S$, one assumes that a "center" item $V^{(i)} \in S$ may predicted the occurrence of
"context" items $V^{(j)}$ which appear in a certain window $W_K(V^{(i)}) = \{ V^{(i+k)} \mid -K < k < K, k \neq 0 \}$
around $V^{(i)}$. Associating every $V \in \mathcal{V}$ with a pair of $d$-dimensional vectors $(v,\bar{v})$ ("center"
and "context" vector), the probabilities $P(V^{(j)} \mid V^{(i)})$ are then modeled via the softmax 
\begin{equation}
\label{eq:P}
    P(V^{(j)} \mid V^{(i)}) = \frac{\exp(v_i^T \bar{v_j})}{\sum_{W}\exp(v_i^T \bar{w}) },
\end{equation}
where the sum in the denominator is taken over all possible items $W$ corresponding to the vectors $(w,\bar{w})$. Maximizing the
logarithm of (\ref{eq:P}) and applying the standard negative sampling technique, which drastically reduces the overall computational
effort, one eventually arrives at the following algorithmic recipe:

\begin{enumerate}
       
\item Initialize all "center" vectors using some random initialization, e.g. by sampling every coordinate uniformly from $[-1/d,1/d]$, and set all "context' vectors to zero.

\item From every sequence $S=(V^{(1)},V^{(2)}, V^{(3)},...)$ choose a number of pairs
    ("skip-grams") $(V^{(i)}, V^{(j)})$  and for every such pair randomly sample $N_{\text{neg}}$ nodes $Q^{(k)}$
        according to a predefined distribution over all nodes. The latter part is commonly referred to as "negative
        sampling", the corresponding distribution is usually named "noise distribution".

\item  For the pairs $(V^{(i)}, V^{(j)})$ together with negative samples  $Q^{(k)}$ compute the loss function
\begin{equation}
\label{eq:loss}
L = -\log \sigma(v_i^T\bar{v_j}) - \sum_{k=1}^{N_{\text{neg}}} \log \left(1-\sigma(v_i^T \bar{q_k})\right),
\end{equation}
compute the gradients $\partial_{v_i} L$, $\partial_{\bar{v_j}} L$, $\partial_{q_k} L$ and apply some variant of Stochastic
        Gradient Descent (usually asynchronous SGD, also known as \textit{Hogwild!} \cite{hogwild}).

\item Repeat Steps 2  to 4 for a number of epochs.
\end{enumerate}
The resulting embedding is usually taken as $f(V) = v$ or sometimes $f(V) = v+\bar{v}$. Concrete algorithms
generally differ in the form of the sequences $S$, the definition of $W_k$, as well as the method of producing negative samples $Q^{(k)}$. 

We now give an informal argument for the effectiveness of this method. For this purpose we first look at the concrete gradients of (\ref{eq:loss}). There, we have
\begin{eqnarray}
\label{eq:grad} 
    \partial_{v_i} L &  =  & (\sigma(v_i^T\bar{v_j})-1) \bar{v_j} - \sum_{k=1}^{N_\text{neg}}  \sigma(v_i^T\bar{q_k})
    \bar{q_k},   \nonumber \\
    \partial_{\bar{v_j}} L &  =  & (\sigma(v_i^T\bar{v_j})-1) v_i,  \\
    \partial_{\bar{q_k}} L &  =  & -\sigma(v_i^T\bar{q_k}) v_i. \nonumber
\end{eqnarray}

\textbf{TODO: The rest of the subsection needs to be rewritten. Not entirely correct}


Thus, since all SGD update steps are of the form
\[
v_i \leftarrow v_i - \eta  \partial_{v_i} L, \quad \bar{v_j} \leftarrow \bar{v_j} - \eta  \partial_{\bar{v_j}} L,
\]
and all $\bar{v_j}$ have been initialized as zero\footnote{This is a typical choice in most implementations.}, it follows that after any number of iterations trained vectors may be written as
\begin{equation}
\label{eq:alphav}
v = \sum_{W \in \mathcal{V}} \alpha(V, W) w_0, \quad \bar{v} =  \sum_{W \in \mathcal{V}} \bar{\alpha}(V, W) w_0
\end{equation}
where $w_0$ is the randomly initialized start vector of the item $W$ and  $\alpha(V, X)$ and $\bar{\alpha}(V, X) \in \mathbbm{R}$ are roughly proportional to the co-occurrence of $V$ and $X$, i.e. in expectation there should hold $\alpha(V, X) < 0$, if $V$ and $X$ never occurred in the same context and $\alpha(V, X) > 0$, if $V$ and $X$ occurred in the same context (This is a direct consequence of the form of the SGD iteration and the fact that $0 < \sigma < 1$). \\

Hence, taking any two trained vectors $v$ and $w$, their scalar product may be expressed as
\begin{eqnarray*}
v^T w & = & \left(\sum_{X \in \mathcal{V}} \alpha(V, X) x_0\right)^T   \left(\sum_{Y \in \mathcal{V}} \alpha(W, Y) y_0\right)  \nonumber \\
          & = & \sum_{X \in \mathcal{V}}  \sum_{Y \in \mathcal{V}} \alpha(V, X) \alpha(W, Y) x_0^T y_0,
\end{eqnarray*}
For sufficiently large $d$, we may assume that the scalar product of two uniformly distributed unit norm random vectors $v$ and $w$ in $\mathbbm{R}^d$ is approximately distributed as $N(0,1/d)$. This allows us to simplify the last expression as
\begin{equation}
\label{eq:approxsimilarity}
v^T w \approx \sum_{X \in \mathcal{V}}  \alpha(V, X) \alpha(W, X) \underbrace{x_0^T x_0}_{\approx 1}.
\end{equation}
This implies, that  $v^T w$ should be positive for items $V$ and $W$ which frequently co-occur in the same context window, or if both co-occur in other items' contexts. Vice versa, $v^T w$ will be smaller or even negative if $V$ and $W$ never co-occurred, since in this case they only enter the SGD iteration as negative samples. 

%The asymptotic point of view also allows us to shed some more light on the $\alpha$ term: In \cite{levygoldberg} Levy and Goldberg show that for a maximizer of the loss (\ref{eq:loss}) and sufficiently large $d$ there holds 
%\[
%v^T \bar{w} = \text{PMI}(V,W) - \log (k).
%\]
%Under the additional assumption that all initial vectors have unit length and $\alpha(V, W)$, $\bar{\alpha}(V, W)$ converge to 
%$\alpha^{*}(V, W)$, $\bar{\alpha}^{*}(V, W)$ we rewrite this as 
%\[
%v^T \bar{w} = \sum_{X \in \mathcal{V}}  \alpha^{*}(V, X) \bar{\alpha}^{*}(W, X) = \text{PMI}(V,W) - \log (k),
%\]
%which implies \textbf{TODO: wrong?}
%\[
%\alpha^{*}(V, W) = \frac{ \text{PMI}(V,W) - \log (k)  - \sum_{X \neq W }  \alpha^{*}(V, X) \bar{\alpha}^{*}(W, X)}{\bar{\alpha^{*}}(W, W)},
%\]
%showing that $\alpha(V, W)$ is indeed approximately proportional to $\text{PMI}(V,W)$. 

%We can now shed some more light on the role of $\alpha$ and $\bar{\alpha}$. To this end, we define the $N$ by $N$ matrix $A$ via $A = ( \alpha(V,W) )_{V,W \in \mathcal{V}}$ and $\bar{A}$ via 
%$\bar{A} = ( \bar{\alpha}(V,W) )_{V,W \in \mathcal{V}}$, so that we can rewrite (\ref{eq:alphav}) in matrix form as
%\begin{equation}
%\label{eq:matrix}
%\boldsymbol{V} = A(\mathcal{V}) \boldsymbol{V}_0, \quad \boldsymbol{\bar{V}} = \bar{A}(\mathcal{V}) \boldsymbol{V}_0.
%\end{equation}
%Here $\boldsymbol{V}_0$ denotes the matrix whose rows are formed by the initial vectors $v_0$ and $\boldsymbol{V}$, $\boldsymbol{\bar{V}}$ the matrices formed by the embeddings $v$, resp. $\bar{v}$. 
%Now, following the argument presented by Levy and Goldberg in \cite{levygoldberg}, we see that in the limit there must hold
%\[
%A(\mathcal{V}) \bar{A}(\mathcal{V})^T = \text{PMI} - \log (k),
%\]
%if $d = N$ and the initial vectors $\boldsymbol{V}_0$ form an orthonormal basis of $\mathbbm{R}^N$.

%Overall, this admits an intruiging interpretation: If we go back to the case $d << N$, then we can interpret the initial data $\boldsymbol{V}_0$ in  (\ref{eq:matrix}) as a random projection from $\mathbbm{R}^N$ into $\mathbbm{R}^d$, mapping rows of the matrices  $A(\mathcal{V})$ and $\bar{A}(\mathcal{V})$ into a low dimensional vector space. Thus, we arrive at the following conclusion: \textit{Embeddings obtained using Skipgram with Negative Sampling can be interpreted as a random projection of high-dimensional, sparse co-occurrence vectors into a lower dimensional space, where representations are dense.} 

We acknowledge that the above results are rather informal and encourage a more rigorous treatment by the community.

%The projection interpretation of SGNS immediately suggests the following:
%\begin{enumerate}
%\item Initial vectors should be "as orthogonal" as possible?
%\item Initial vectors should be initialized to unit length?
%\end{enumerate}

%If we have an explicit expression of alpha in terms of pmi then we can deduce a simple incremental training scheme.'

%What do the alphas converge to?






\subsection{Adding Side Information}
In the context of recommender systems it seems natural to extend the SGNS-type embedding approach beyond the simple usage of item
co-occurrences. A natural extension is provided by incorporating item features. More concretely, assume that every item
$V=(V_1,...,V_{M})$ is determined by $M$  integer features, each belonging to one of $m$ "feature columns", e.g. "Column
0 = Shop", "Column 1 = Age", "Column 2 = Category", etc.  For every such column we may then, in addition to every item,
also embed every possible feature value (e.g. "Leaf Category = Women's Sports Shoes" or "Age = 19-21") as a vector in
$\mathbbm{R}^d$.  For the feature vector corresponding to the $i$-th feature $V_i$ of an item $V$ we will then write
$s_i(V)$ and call such a vector "side information vector". The number of all such vectors (or equivalently distinct
feature values) will be denoted by $N_s$. Note that if $V_i=U_i$ for two items $U$ and $V$, then $s_i(V)=s_i(U)$.

A number of authors have proposed ways of incorporating side information into a graph embedding models. In \cite{EGES}
two of the authors of this article have proposed to substitute the single item vector $v$ of $V$ with a linear combination of an "item"
vector $v_0$ and its side information vectors $s_i(V)$. All item, side information vectors and weights are then learned
together. 

Alternatively, a different approach has been proposed under different names in \cite{mp2v}, \cite{alikdd2},
\cite{metapath2vec}, \cite{starspace} and \cite{airbnb}. Up to minor difference it can be summarized as follows:
Sequences of items are substituted by sequences of item and side information features and the "enriched"
sequences are then again fed into an SGNS-type embedding algorithm. Thus, an embedding for both the vectors $v$ and
$s_i(V)$ is learned at the same time. In the following we will refer to such approaches using the term "context enriched SGNS-type embedding
algorithms". From the NLP/word embedding point of view this could be interpreted as a joint embedding of words and sentence topics (See e.g.
\cite{topical}).

As an example, assume that every item belongs to one category, such as for instance "Women's Sports Shoes" or
"Electronics". Then, the sequence 
\begin{quote} \texttt{Item\char`_1} \texttt{Item\char`_2} \texttt{Item\char`_3} ... \end{quote}
could be enriched by adding each item's category after the item itself:
\begin{quote} \texttt{Item\char`_1} \texttt{Item\char`_1\char`_Category} \texttt{Item\char`_2}
    \texttt{Item\char`_2\char`_Category} \texttt{Item\char`_3} \texttt{Item\char`_3\char`_Category} ... \end{quote}
Alternatively, one could obtain an embedding only for categories via
\begin{quote} \texttt{Item\char`_1\char`_Category} \texttt{Item\char`_2\char`_Category}
\texttt{Item\char`_3\char`_Category} ... \end{quote}

Clearly, this procedure has two main advantages: First, it may be used in conjunction with any standard word embedding
implementation, and secondly it is flexible enough to be used in a wide number of different recommendation domains.  We
will present a concrete application this approach in the following section. We believe that this approach provides for a good trade-off between model flexibility, accuracy and real-world
usability in production environments. As an example outlining the flexibility of this approach we mention the recent
paper \cite{airbnb}, in which the authors have explored this approach in a similar setting. A promising idea of theirs
is to enrich sequences not only with side information but also specially crafted item- and user types, as well as by adding
items, that were actually bought into the final sequences. 

The idea of  context enrichment has been applied in an ad-hoc manner by a number of authors who have reported significant increases in overall model performance. However, we are not aware of a satisfactory theoretical explanation for the increased performance of this approach. We hence address this issued in the remainder of this subsection.

Consider for example two items $V$ and $W$ with trained embeddings $u$ and $v$. Using (\ref{eq:approxsimilarity}) we find that
\[
v^T w \approx \sum_{X \in \mathcal{V\setminus S} } \alpha(V, X) \alpha(W, X) x_0^T x_0 + \sum_{S \in \mathcal{S}}  \alpha(V, S) \alpha(W, S) s_0^T s_0,
\]
where $\mathcal{S} \subset \mathcal{V}$ denotes the set of all  "side information nodes". Now, if $V$ and $W$ never occur together in a common context (i.e. the same window) the first sum will be small or possibly negative. However, if both $V$ and $W$ share some side information $S$, then $\alpha(V, S)$ and $\alpha(W, S)$ should both be larger than $\alpha(V, T)$ and $\alpha(W, T)$ for some side information $T$ not belonging to $V$ and $W$, if $S$ has been added into the training sequences in all windows context windows containing either $V$ or $W$. Thus, using the context enrichment procedure, we achieve on average a higher similarity for those items which have the same side information, even if the items themselves do not occur in the same context.

%Scalability
\subsection{Scaling SGNS-type Algorithms}
\label{sect:scaling}
As we have seen, basic SGNS-type embedding algorithms such as word2vec may be applied in  straight forward manner in to
obtain joint item and side information embeddings used for recommendation systems. There remains, however, an important
challenge: Scaling this approach to very large, that is possibly billion-scale, datasets. While this might seem
unrealistic at first, we note that the number of all available products on Taobao already exceeds the 500 million mark
by a significant margin. We are thus dealing with a real-world application scenario.

In a single machine / shared memory setting SGNS-type algorithms are generally trained using asynchronous
(\textit{Hogwild!}) SGD
\cite{hogwild}, such that embedding vectors are shared among all threads. Possibly conflicting updates from different
threads are ignored. Most implementations ignore the possibility of conflicting memory updates, since such events are rather improbable when dealing with larger sized graphs. They may nevertheless have an impact on performance \cite{collision}. 

Clearly, such an approach is difficult to implement in a distributed computing environment. However, there exist a number of methods to deal with such a situation. The simplest approach, as outlined for instance in \cite{pword2vec} is to adopt a data parallelism strategy, which amounts to replicating all embedding vectors on every worker node and then synchronizing the trained model updates using either simple averaging after a number of time steps or utilizing a parameter server. Either way, the entire model, that is all embedding vectors and other parameters have to be stored in at least one machine's memory.

Smarter approaches have been proposed in \cite{dsgns} and \cite{ordentlich}. In \cite{ordentlich} the problem is
approached via sharding of the embedding vectors by dimension rather than nodes. The proposed architecture makes use of
two kinds of workers: the first kind, resembling parameter servers, stores shards of the embedding vectors, such that
each worker of this kind only contain a fixed number of coordinates $p < d$ for all nodes.  The second kind of workers
("clients") independently sample skip-grams and send each pair to all parameter servers, which then compute partial scalar products of the embedding vectors. The partial scalar products are returned to the clients, aggregated, and finally sent back to the parameter servers where they are used to perform updates using (partial) gradients.

\textbf{TODO: mention swivel}

The method described in \cite{dsgns} constitutes another intriguing solution using an algorithm called "Target Negative
Sampling" (TNS). In this approach, all items (words, graph nodes, resp.) are split into several partitions. Each worker
then stores only the embedding vectors of items belonging to its partition. In contrast to most single machine SGNS
implementations, all workers then sample skip-grams from the entire corpus.

If both center and context word are maintained by a single worker, then a local gradient update is performed immediately. If Worker A samples a skip-gram such that the center word is not maintained by Worker A, the skip-gram will be ignored. If the center word is maintained by Worker A and the context word by Worker B, then Worker A will send the corresponding center vector to Worker B. Upon receiving the vector from Worker A, Worker B computes the gradients of the loss function (\ref{eq:loss}) while sampling negatives only from its local partition. After updating the context vectors in its local partition, the gradient of the center vector is returned to Worker A, which then updates the corresponding center vector.

Motivated by the promising results reported in \cite{dsgns} we have implemented the TNS method in the "Behemoth" proprietary graph embedding platform developed at Alibaba. In the following section we will now describe the details of a concrete context enriched SGNS-type algorithm that we have deployed in production at Taobao.

\section{Context Enriched SGNS for Product and Side Information Embedding}
\label{sect:asymp2v}

For a sequence of items $S = (V^{(0)}, V^{(1)}, V^{(2)}, \ldots) \in \mathcal{S}$ we can model the context enrichment procedure using a mapping $F: \mathcal{S} \rightarrow \mathcal{S}$, so that every choice of $F$ corresponds to a different embedding model. As an example, we can describe the full Meta-Prod2Vec model ("MP2V") via the function
\begin{equation}
\label{eq:fullmp2v}
F(S) = (V^{(0)}, V_1^{(0)}, V_2^{(0)}, \ldots , V_{N_s}^{(0)}, V^{(1)}, V_1^{(1)}, V_2^{(1)}, \ldots , V_{N_s}^{(1)}, \ldots  ),
\end{equation}
which means that in every sequence after every item we add that item's side information. Clearly, this leads to a massive increase of the corpus size. To counter this problem, we may for example modify the transformation $F$ and only add the first item's side information:
\begin{equation}
\label{eq:asymp2v}
F(S) = (V^{(0)}, V_1^{(0)}, V_2^{(0)}, \ldots , V_{N_s}^{(0)}, V^{(1)}, V^{(2)}, \ldots  ) 
\end{equation}
We will call the model trained on these sequences ASYMP2V ("asymmetric Meta-Prod2Vec"). This represents the main model that we have been using daily in our production system. Based on our previous experiences with the EGES model \cite{EGES}, we train the ASYMP2V model with the following side information columns: Shop, Brand, Gender, Style, Color, Age group, Leaf category, Top level category. The item sequences in the ASYMPV model thus take the following form:
\begin{quote} \texttt{Item\char`_1} \texttt{Item\char`_1\char`_Shop} \texttt{Item\char`_1\char`_Brand} 
\texttt{Item\char`_1\char`_Gender} \\ \texttt{Item\char`_1\char`_Style} \texttt{Item\char`_1\char`_Color}
    \texttt{Item\char`_1\char`_Age} \\ \texttt{Item\char`_1\char`_LeafCategory} \texttt{Item\char`_1\char`_TopLevelCategory}
    \texttt{Item\char`_2}
    \texttt{Item\char`_3} ... \end{quote}

In this article we will also be exploring the effect of other choices for $F$. Consider for instance the transformation
\begin{equation}
\label{eq:smp2v}
F(S) = \text{Shared}(S) \cup (V^{(0)}, V^{(1)}, V^{(2)}, \ldots), 
\end{equation}
where $\text{Shared}(S)$ is the set of all the side information features shared by all elements in the sequence $S$. We can extend this further using
\begin{equation}
\label{eq:sump2v}
\begin{aligned}
F(S) = \text{Shared}(S) \cup ( & V^{(0)}, \text{Unique}(S, V^{(0)}), V^{(1)}, \text{Unique}(S, V^{(1)}), \\  &   V^{(2)},  \text{Unique}(S, V^{(2)}), \ldots),
\end{aligned}
\end{equation}
which amounts to extending (\ref{eq:smp2v}) with the addition of the remaining features while avoiding duplicate elements per transformed sequence. 

We will report the effect of the particular choice of $F$ later in Section (\ref{s:cases}). In our setting, however, the effects of different choices of $F$ have shown to be relatively minor. As a consequence, our standard choice of model has become the ASYMPV model (\ref{eq:asymp2v}), since it provides for a more than decent trade-off between recommendation performance and computational efficiency. We speculate that the observed minor differences between  ASYMP2V and alternatives are mainly due to the fact that 
Taobao users on average tend to successively view items with very similar side information. In particular, it is rare for users to switch to a different leaf category within one browsing session.
\textbf{TODO: Possibly change these statements after results for all experiments are there.}


\subsection{Context-Enrichment and TNS}
\label{sect:asymp2vtns}
Clearly, since some of the side information columns might contain only a small number of distinct feature values
(e.g. "Gender" takes only three  values: "female", "male", "null"), the total corpus of item sequences will suffer from
a highly imbalanced distribution of "word" frequencies. As is normal in the context of distributed algorithms, this can
have a negative impact on the performance of our TNS-based embedding algorithm. We have addressed this problem in two ways:
\begin{itemize}
    \item High frequency objects are aggressively down sampled.
    \item Our implementation of TNS allows for the top-K frequency items to be kept in all partitions at the same time.
        The corresponding vectors are then synchronized (averaged) at regular intervals. We have thus implemented a
        hybrid TNS/model averaging based strategy.
\end{itemize}

In addition to the frequency imbalance, we would like to discuss a further point, that is relevant to the scalability of
the ASYMP2V/TNS combination: Since pairs of center and context items are sent to another worker node for processing, if
the context word is not managed by the worker which has sampled this pair, it is obvious that a completely randomized
partitioning strategy may lead to a massive performance reduction. To counter this problem, we have implemented heuristic balanced graph partitioning strategy. We describe this strategy and the details of our TNS implementation in the following two subsections.

\subsection{Efficient Distributed Training using Hybrid TNS}
We now describe in detail how to address the algorithmic challenges outlined in the previous section. Before the actual training algorithm starts, a number of preprocessing steps have to be performed:
\begin{enumerate}
\item Transform all item sequences $\mathcal{S}$ into $\tilde{\mathcal{S}} = F(\mathcal{S})$ using the sequence enrichment function $F$.
\item Count item and side information frequencies in  $\tilde{\mathcal{S}}$, so that we obtain a dictionary $\mathcal{D}$  containing all item and side information IDs, as well as frequencies.
\item Partition $\mathcal{D}$  into $(\mathcal{P}_1, \mathcal{P}_2, \ldots, \mathcal{P}_w)$, where $w > 0$ denotes the number of workers. The target partition for item nodes (i.e. products) is determined according to a user supplied partitioning strategy, while target partitions for side information nodes are assigned randomly.
\item Determine the set of shared nodes $\mathcal{Q}$ containing all elements (items or side information) of $\mathcal{D}$ with a frequency above a certain threshold. In our setting, this this has the effect of $\mathcal{Q}$ containing the most common side information features such as age, gender, color, etc.
\end{enumerate}
The actual training process is then performed according to Algorithm \ref{alg:tns}.  

\begin{algorithm}[h]
 \KwData{List of item sequences $\mathcal{S}$, List of shared items $\mathcal{Q}$, WorkerID, Partition $P_\text{WorkerID}$, Dictionary $D$,  sequence enrichment function $F$, learning rate $\eta$, synchronization period $t_\text{sync}$}
 %\KwResult{how to write algorithm with \LaTeX2e }
 j := Worker ID\;
 t := 0\;
 Initialize all vectors for $\mathcal{P}_j \cup \mathcal{Q}$\;
 Build a local noise distribution for all elements in $\mathcal{P}_j \cup \mathcal{Q}$ utilizing frequencies from $D$\;
 Barrier\;
 \For{$S \in \mathcal{S}$ }{
 
  \For{ each pair $(V,W)$ sampled from $S)$}{
 
    \If{ $\mathcal{P}_V \notin \mathcal{P}_j$ and $\mathcal{P}_W \notin P_j$ } {   
    continue\;
  	}
  
    \If{ $\mathcal{P}_V \notin \mathcal{P}_j$ and $\mathcal{P}_W \in \mathcal{P}_j$ } {   
 	   continue\; 
	  }
  
    $\partial_v L$ := Call TNS($V$,$W$) on worker $\mathcal{P}(W)$ \;
    $v$ :=  $v - \eta \partial_v L$ \;
  
    t := time()\;
    \If{time() - t >  $t_\text{sync}$}{
    	 Barrier\;
	 Average vectors across all workers for all $Q \in \mathcal{Q}$  \;
	 t := time()\;
    }
   }
 }
\BlankLine
\BlankLine

 \SetAlgoLined
\SetKwProg{Fn}{Function}{}{end}
\Fn{TNS($V$,$W$)}{

Sample negatives $Q^{(k)}$ from the local noise distribution\;
Compute $\partial_{v} L$, $\partial_{\bar{w}}$, $\partial_{\bar{q_k}}$ according to Eq. (\ref{eq:grad})\;

$\bar{w}$ :=  $\bar{w} - \eta \partial_{\bar{w} }L$ \;
\For{each negative sample $Q^{(k)}$} {
$\bar{q}_k$ :=  $\bar{q}_k - \eta \partial_{\bar{q}_k} L$ \;
}

return $\partial_{v} L$\;
}
\caption{Hybrid TNS} \label{alg:tns}
\end{algorithm}

Besides the graph partitioning strategy, which will be described in the next subsection, it remains to mention the implementation details regarding pair sampling and generation of negative samples:
\begin{itemize}
\item We have implemented sampling of pairs $(V,W)$ following the standard word2vec implementation, that is  based on selecting context items using a window around the center item with a fixed window size. Since all of our training sequences are of the same length, we can adjust the window size, such that all possible pairs per sequence are sampled.
\item We also apply the same method of subsampling very frequent pairs as proposed originally in \cite{word2vec}. In our setting, which is characterized by a number of very high frequency objects due to the additional side information it has been proven practical to aggressively downsample high-frequency pairs. To that end we typically choose the sample parameter as $10^{-5}$.
\item Every worker maintains its own noise distribution for the elements of $\mathcal{P}_j \cup \mathcal{Q}$, where the probability of drawing  $V$ as a negative sample is modeled such that
\[
P_{\text{noise}}(V) \sim \text{freq}(V)^\alpha,
\]
where we used the standard choice of $\alpha = 0.75$.
\end{itemize}

\subsection{Heuristic Balanced Graph Partitioning}
Taking a closer look at Algorithm \ref{alg:tns}, it is clear that the overall computational performance will depend on the number of remote calls of $TNS(V,W)$. To keep this number as small as possible, the partitions $\mathcal{P}_i$ have to be cut such that both $V$ and $W$ are managed by the same worker as often as possible. Moreover, sizes of all $P_i$ should be as similar as possible. Since most Taobao users tend to view items from only leaf category within one browsing session, the obvious choice for a partitioning strategy is to define partitions along leaf categories. However, the number of Taobao leaf categories is in general larger than the number of available workers. Moreover, the distribution of the number of items per leaf category may vary greatly. We thus have to properly balance the assignment of leaf categories to worker partitions.

To achieve a balanced assignment we have used the following heuristic balanced graph partition strategy (See Figure \ref{fig:hbgp}):
\begin{enumerate}
\item Estimate the transition probabilities $p(U,V)$ for the i2i-graph G.
\item Reduce the i2i-graph $G$ to a graph $\tilde{G} = (\tilde{\mathcal{V}}, \tilde{\mathcal{E}})$ containing only leaf-category nodes. Assign transition probabilities between category nodes by aggregating probabilities corresponding to edges of $G$ which connect nodes of different leaf categories. Moreover, for $C \in \tilde{\mathcal{V}}$ let $|C|$ denote the number of items from $G$ which belong to category $C$.
\item Iteratively merge nodes of $\tilde{G}$: 
\begin{enumerate}
\item Find the edge $(C_1, C_2)$ with the highest transition probability. 
\item Merge $C_1$ and $C_2$, if  $|C_1|+|C_2| \leq \beta \cdot |\mathcal{V}| / w $, where $\beta \geq 1$ is a user supplied parameter specifying the maximally allowed imbalance. Otherwise repeat this process for the remaining edges ordered by the corresponding transition probabilities until $|C_1|+|C_2| \leq \beta \cdot |\mathcal{V}| / w $ is satisfied. If $|C_1|+|C_2| \leq \beta \cdot |\mathcal{V}| / w $ holds for none of the edges, increase $\beta$ and restart.
\item After merging  $C_1$ and $C_2$ recalculate all transition probabilities accordingly.
\item Repeat until $\tilde{G}$ only consist of $w$ nodes.
\end{enumerate}
\end{enumerate}
Keeping track of which nodes of the category graph are merged, we thus obtain our final partitions $\mathcal{P}_i$. As the above strategy requires careful manual tuning of the parameter $\beta$, we do not fully automate this process in our production system. Moreover, 
for products on the Taobao mobile app, relative sizes of item leaf categories vary very little over periods of several months. In our case, It is thus unnecessary to rebalance partitions more than a few times per year.

\begin{figure*}[hbpt]
\center
\includegraphics[width=0.75\textwidth]{figures/graph_partition.png}
\caption{Heuristic Balanced Graph Partitioning}
\label{fig:hbgp}
\end{figure*}

Using the above strategy we were able to achieve an overall performance gain of roughly 130\% when compared to a purely random assignment of items to partitions. We report some more concrete figures in Section \ref{s:cases}.


\subsection{Notes on Production Deployment and Implementation Details}
In our current production environment we have implemented Context enrichment and generation of the dictionary $\mathcal{D}$ are  as straight-forward Map-Reduce jobs.
 Algorithm \ref{alg:tns} itself has been realized on top the "Behemoth" proprietary graph processing platform. 
In order to ensure maximum efficiency Behemoth has been implemented from the ground up in C++11. Behemoth workers are orchestrated using MPI and most intra-worker communication is realized in an asynchronous manner using several queues per worker. 

All workers run a number of "sampler", "trainer" and "updater" threads in parallel. Sampler threads read input sequences from a distributed file system and then pass on pairs of center and context items to the trainer threads on those workers which maintain the context items. In our implementation we have decoupled gradient calculation from the actual SGD updates, that is gradients computed in the $TNS$ function in  Algorithm \ref{alg:tns}  are received asynchronously via a separate queue, which is read by one of the updater threads on the worker having originally requested this gradient. In our experience, the impact of these delayed gradient updates, appears to be negligible, as long as partitions are balanced.After the embedding calculation item to item similarities are computed and uploaded back into our online systems. For this task we utilize a custom graph-based KNN algorithm which has been directly integrated into the Behemoth platform.

Overall, this setup allows us to compute embeddings and item to item similarities for several hundreds of millions of items in a matter of hours, with all item and side information vectors lying the same semantic vector space. Moreover, since our method does not require all embedding vectors to be kept in every worker's main memory, there is no need to process subgraphs individually. We will report some performance statistics of our system in Section \ref{sect:performance}.

\section{Numerical Experiments and Case Studies}
\label{s:cases}
For the case studies presented in this article we have used the following datasets:
\begin{itemize}
\item TODO
\end{itemize}

Moreover, the following algorithms have been evaluated on the above datasets and compared each other:
\begin{itemize}
\item TODO
\end{itemize}

The parameter settings for all of our experiments are shown in Table X \textbf{TODO}.

\subsection{Evaluation Metric}
To evaluate the different algorithms we use the standard Hitrate@K metric. In our concrete setting this amounts to the following procedure
\begin{enumerate}
\item Take all of user item interactions of the form
\[
\text{Item}_1 \rightarrow \text{Item}_2 \rightarrow \ldots \rightarrow \text{Item}_T
\]
and split them into training sequences consisting of the first $T-1$ items 
\[
\text{Item}_1 \rightarrow \text{Item}_2 \rightarrow \ldots  \rightarrow \text{Item}_{T-1}
\]
and corresponding "labels" given by all $\text{Item}_{T}$.
\item Generate embeddings using the training sequences.
\item Use the embeddings to compute the $K$ most similar items for each $\text{Item}_{T-1}$ and compute  Hitrate@K via
\[
\text{HR@K} = \frac{\#\text{(Item}_T \text{ appears in K most similar items)}}{\#\text{(total number of training sequences)}}
\]
\end{enumerate}
For our experiments we have computed similarities using the standard cosine similarity.

\subsection{Training Parameters and Implementation Details} In the following we briefly describe here the parameter settings that we have used during our experiments. For all experiments we choose $d=160$ as the embedding space dimension and train for $k=2$ epochs using $N_{\text{neg}}$ negative samples. 

\subsection{Results for Dataset X} 
We report the resulting hit rates for the proposed algorithms in Table 
 
\subsection{Results for Dataset Y} 
We report the resulting hit rates for the proposed algorithms in Table 

\subsection{Cold Start Items and other Transfer Tasks}
\label{sect:coldstart}
We briefly sketch how ASYMP2V deals with the problem of cold start recommendation for new
items: Suppose that we are given a new item $V$, for which there exists no data relating it to other items and hence no
embedding vectors. Heuristically, it would make sense to "infer" and embedding vector $v$  for $V$ via
\begin{equation}
\label{eq:coldstart}
v = \sum_{k=1}^{M}  s_k(V),
\end{equation}
with $s_k(V)$ obtained from a previous training run. Equation (\ref{eq:approxsimilarity}) again allows us to justify this approach: Writing a single side information vectors as
\[
s_k(V) = \sum_{W \in \mathcal{V}} \alpha(W, V_k) w_0
\]
we obtain
\begin{eqnarray*}
w^T v  & \approx &  \sum_{k=1}^{M}  \sum_{X \in \mathcal{V}} \alpha(W, X)  \alpha(V_k, X)  \nonumber \\ 
& = &   \sum_{k=1}^{M}  \left( \sum_{X \in \mathcal{V} \setminus \{V_1, \ldots, V_k  \}} \alpha(W, X)  \alpha(V_k, X) +   \sum_{j=1}^{M}  \alpha(W, V_j)  \alpha(V_k, V_j)   \right). \nonumber
\end{eqnarray*}
This implies that $V$ should be more similar to those items $W$ which frequently occur with the side information nodes $V_k$.

In Figure \ref{fig:coldstart} we give an example for cold-start recommendations obtained via (\ref{eq:coldstart}). To produce this example, we have trained an ASYMP2V model on user generated sequences for roughly 80 million items on Taobao and then performed 
KNN queries using the regularly trained vector $v$ and the approximation (\ref{eq:coldstart}) as input for the query.

\begin{figure*}[hbpt]
\center
\includegraphics[width=0.75\textwidth]{figures/coldstart.pdf}
\caption{Example: ASYMP2V cold start recommendation }
\label{fig:coldstart}
\end{figure*}

\subsection{Online Evaluation during 2018 11.11 Global Shopping Festival}
TODO

\section{Discussion and Related Work}
TODO

\subsection{Recommendation Performance}
TODO

\subsection{Computational Performance}
\label{sect:performance}
TODO.

\section{Summary}
TODO

